Failure-Resilient Coverage Maximization with Multiple Robots

The task of maximizing coverage using multiple robots has several applications such as surveillance, exploration, and environmental monitoring. A major challenge of deploying such multi-robot systems in a practical scenario is to ensure resilience against robot failures. A recent work introduced the Resilient Coverage Maximization (RCM) problem where the goal is to maximize a submodular coverage utility when the robots are subject to adversarial attacks or failures. The RCM problem is known to be NP-hard. In this paper, we propose two approximation algorithms for the RCM problem, namely, the Ordered Greedy (OrG) and the Local Search (LS) algorithm. Both algorithms empirically outperform the state-of-the-art solution in terms of accuracy and running time. To demonstrate the effectiveness of our proposed solution, we empirically compare our proposed algorithms with the existing solution and a brute force optimal algorithm. We also perform a case study on the persistent monitoring problem to show the applicability of our proposed algorithms in a practical setting.

==> 2_related_works.tex <==
\section{Related Works}
\label{rw}

The existing work by Lifeng is called \textit{2PG} algorithm (2 Phase Greedy algorithm). 

todo

==> 4_oblivious_greedy.tex <==
\section{Oblivious Greedy Algorithm}
\label{obg}

In this section, we present a straightforward algorithm for the resilient coverage maximization problem. The algorithm selects, for each robot, the trajectory that covers maximum number of targets. Formally, the solution found by this algorithm is $\bigcup_{r \in \mathcal{R}} \argmax_{\tau \in \mathcal{T}_r} {\rm F} (\{ \tau \})$. We call this algorithm the Oblivious Greedy Algorithm (\textit{ObG}). \textit{ObG} makes $P$ calls to the target coverage function F. Recall from Section~\ref{pf} that, $P$ is the sum of number of trajectories of all robots. 
